The Rainbow Skip Graph: A Fault-Tolerant Constant-Degree P2P Relay Structure

We present a distributed data structure, which we call the rainbow skip graph. To our knowledge, this is the first peer-to-peer data structure that simultaneously achieves high fault tolerance, constant-sized nodes, and fast update and query times for ordered data. It is a non-trivial adaptation of the SkipNet/skip-graph structures of Harvey et al. and Aspnes and Shah, so as to provide fault-tolerance as these structures do, but to do so using constant-sized nodes, as in the family tree structure of Zatloukal and Harvey. It supports successor queries on a set of n items using O(log n) messages with high probability, an improvement over the expected O(log n) messages of the family tree.

==> ErasureSummary.tex <==
An $(n,c,l,r)$-erasure-resilient code consists of an encoding algorithm
and a decoding algorithm.  The encoding algorithm takes a message of
$n$ bits and converts it into a sequence of $l$-bit packets whose total
size is $cn$ bits.  The decoding algorithm is able to recover the
original message from any set of packets whose total length is $rn$.
Alon and Luby~\cite{alon96linear} 
provide a deterministic $(n,c,l,r)$-erasure-resilient
code with linear-time encoding and decoding algorithms with $l=O(1)$.
Although these codes are not generally the most practical, they give
the most desirable theoretical results.  
%It is worth noting that since
%our model considers only the message complexity, we needn't necessarily
%choose to use a linear-time code; we do so merely for the added comfort
%of maintaining efficient usage of computational power.

